Heuristic-based Mining of Service Behavioral Models from Interaction Traces

Software behavioral models have proven useful for emulating and testing software systems. Many techniques have been proposed to infer behavioral models of software systems from their interaction traces. The quality of the inferred model is critical to its successful use. While generalization is necessary to deduce concise behavioral models, existing techniques of inferring models, in general, overgeneralize what behavior is valid. Imprecise models include many spurious behaviors, and thus compromise the effectiveness of their use. In this paper, we propose a novel technique that increases the accuracy of the behavioral model inferred from interaction traces. The essence of our approach is a heuristic-based generalization and truthful minimization. The set of heuristics include patterns to match input traces and generalize them towards concise model representations. Furthermore, we adopt a truthful minimization technique to merge these generalized traces. The key insight of our approach is to infer a concise behavioral model without compromising its accuracy. We present an empirical evaluation of how our approach improves upon the state-of-the-art specification inference techniques. The results show that our approach mines model with 100% precision and recall with a limited computation overhead.

==> abstract.tex <==
\begin{abstract}
\label{sec:abstract}

Software behavioral models have proven useful for emulating and testing software systems. Many techniques have been proposed to infer behavioral models of software systems from their interaction traces. The quality of the infer model is critical to their successful use. While generalization is necessary to deduce behavioral models concisely, existing techniques to infer models, in general, overgeneralize what behavior is valid. Imprecise models include many spurious behaviors, and thus compromise the quality of techniques that use those models.

In this paper, we propose a novel technique that increases the precision of the behavioral model represented as automata inferred from interaction traces. The essence of our approach is heuristic-based generalization and truthful minimization. The set of heuristics include patterns to match against input traces to generalize them towards model representation. We adopt a truthful minimization technique to merge these generalized traces. The key insight of our approach is to infer a concise behavioral model without compromising its precision. We present an empirical evaluation of how our approach improves upon the state-of-the-art specification inference techniques. We have implemented our novel specification mining technique, and make public our implementations, subject libraries, ground-truth models, and experimental data.
\end{abstract}

==> background.tex <==
\section{background}
\label{sec:background}
A Retailer service~\cite{4515865} allows its clients to purchase products and can have two types of clients: regular and premium. A typical conversation of regular clients may start with a request for the product catalog, followed by an order. Then, an invoice is sent to clients, and once the payment has been made, the requested goods will be shipped. For premium customers, goods may be shipped immediately after placing an order (the invoice is sent later). The specification of the Retailer service is depicted in Figure \ref{fig:retailerservice}. In the following, we use shortened forms of these messages for simplicity: regLogin, cata, order, inv, pay, ship for regular customer and  premLogin, cata, order, ship, inv, pay for premium customer. 

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/background}
	\caption{\small{The specification of the \emph{retailer} service}}
	\label{fig:retailerservice}
\end{figure}

==> conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}
To improve precision of the inference FSA from traces, in this paper we propose a heuristic driven technique to generalize system behavior where we start with intra-trace state merging based on a rich set of heuristics that consistently address different types of generalization cases in a FSA. The basis of our heuristics is the system behavior patterns present on the traces which provide us evidences for generalization. We evaluated our technique on a set of systems from various domains that show how our approach can significantly increase precision without loss of recall, and with a limited overhead on the inference process. 

This work is significant as the form of specifications that can be mined are richer than previous approaches. Importantly, this work also lays the foundations for further work allowing us to extend our specification mining technique to the parametric specification.


==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
We empirically evaluated the effectiveness of our approach by comparing the quality of the models learned using SpecMiner with the models learned using kTail and Synoptic. In the following subsections, we describe the data set, the evaluation setup, and finally present the results of our experiments.

\subsection{Subject systems}
We applied SpecMiner in four different systems.

\begin{itemize}
	\item 
	\textbf{Concurrent Versions System (CVS)} is a free software client-server revision control system in the field of software development to keep track of all work and all changes in a set of files, and allows several developers (potentially widely separated in space and time) to collaborate.
	\item
	\textbf{Amazon-ec2} is a commercial web service from Amazon's Web Services (AWS) that lets customers "rent" computing resources from the Elastic Compute Cloud (EC2). It provides storage, processing, and web services to customers.
	\item 
	\textbf{StringTokenizer} is a Java library (\emph{java.util.String- Tokenizer}) for breaking a string into tokens. It is simple way to break string and doesn't provide the facility to differentiate numbers, quoted strings, identifiers etc.
	\item
	\textbf{ZipOutputStream} is a Java library (\emph{java.util.zip.Zip- OutputStream}) for writing files in the ZIP file format, which includes support for both compressed and uncompressed entries.
\end{itemize}

\subsection{Evaluation setup}
In this section, we describe the evaluation metrics, ground-truth models and experimental design.
\subsubsection{Evaluation metrics}
We measured precision, recall and time required to perform the mining as evaluation criteria. \emph{Precision} is the percentage of mined behaviors that are correct, namely the percentage of behaviors generated by the mined model that are accepted by the model to be inferred, i.e., the ground truth model. \emph{Recall} is the percentage of correct behaviors that have been mined, i.e., the percentage of behaviors generated by the model to be inferred that are accepted by the mined model. Since the model can have infinite traces, we restricted the transition visit limit twice for trace generation from infer and ground truth model.

\subsubsection{Ground-truth model}
Evaluating the quality of the inferred models requires a set of ground-truth models that represent the systems' legal behaviors. To this end, we used the ground-truth models that were manually extracted as part of related work~\cite{lo:2009,LO20122063}

\subsubsection{Experimental design}
For each subject system, we inferred four models: traditional kTail with k=1 and k=2, synoptic, and our approach. We do not report results of kTail for k>2 because those k values led to fewer merges, which lowered the recall without notable precision improvement.
In the experiments, for each subject system, we performed three steps: (1) generate input traces from the ground truth model with path coverage where each transition is visited maximum twice, (2) run the four inference algorithms on those input traces, and (3) measure the precision and recall of the inferred models. 

%The implementation, observed traces, inferred models, and ground-truth model are publicly available at \url{http://www.ict.swin.edu.au/personal/akabir/}.

\subsection{Results}
We compare the effectiveness and efficiency of our approach with kTail (k=1 and k=2) and Synoptic by computing the precision and recall for the resulting automata and measuring the time required to generate the models. Table \ref{tab:empiricalresult} shows the results of our experiments.

\begin{table*}[tbh]
	\centering
	\caption{Empirical Result}
	\label{tab:empiricalresult}
	\begin{tabular}{|l|*{13}{c|}}
		\hline
		\multirow{2}{*}{\textbf{Approaches}}
		& \multicolumn{3}{|c|}{\textbf{CVS Client}} 
		&   \multicolumn{3}{|c|}{\textbf{Amazon-ec2}} 
		&   \multicolumn{3}{|c|}{\textbf{StringTokenizer}} 
		&    \multicolumn{3}{|c|}{\textbf{ZipOutputStream}}\\
		\cline{2-13} & P & R & T & P & R  & T & P & R & T & P & R & T \\ \hline
		
		kTail, k=1 &0.0022 & 0.528 & 68 & 1 & 1 & 147 & 1 & 1 & 19 & 1 & 1 & 47  \\\hline
		kTail, k=2 & 1 & 0.339 & 90 & 1 & 0.346 & 120 & 1 & 1 & 15 & 1 & 1 & 34  \\ \hline
		Synoptic & 0.244 & 1 & 396 & 1 & 1 & 373 & 1 & 1 & 611 & 1 & 1 & 337  \\\hline
		Our approach &  1 & 1 & 47 & 1 & 1 & 65 & 1 & 1 & 43 & 1 & 1 & 99  \\ \hline
		\multicolumn{13}{l}{\textsuperscript{*}Note: P is precision, R is recall, and T is time in milliseconds.}
	\end{tabular}
\end{table*}
%CVS 130
%ec2 485

The results show that the precision of the models inferred by our approach is significantly higher than the precisions of the models inferred by other approaches. We observed the highest difference in precision when experimenting with CVS client system. In this the case, given the best recall (i.e., 1), the precision of the inferred model raises from 0.244 in the case of model inferred by Synoptic, to 1 in the case of model inferred by our approach. It is worth to noticing that in this study our approach always generated models with perfect precision (i.e., 1). Even for some other subjects such as StringTokenizer and ZipOutputStream, Synoptic also inferred models with perfect precision, our approach takes less time compare to Synoptic to infer models with same precision. The data reported in Table \ref{tab:empiricalresult} shows that our approach most efficiently infer models with better precision and no loss of recall. 



==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Behavioral models capture behaviors that software systems obey. They play an integral role in software design, validation, verification, maintenance and testing [].They can help to verify the software implementation [] and guide test case generation to improve test coverage []. In software maintenance, behavioral models assist engineers to understand the complex objects and their interactions [], as well as support debugging, fault detection, and detecting other anomalies []. In enterprise software testing environament, behavioral models aid to emulate services by synthesizing service response messages from models [].

Despite its high importance in software development process, a formal/abstract model of the software behavior is often missing or incomplete. Although several systems that follow recommended requirements gathering and design practises during early stages, they deviate from their early specifications as development and maintenance progresses. This deviation leads to inject errors in the implementation and changes in the requirements themselves. As a result, even if a software specification is available - it may not reflect the behaviors of the latest version of the software.

Numerous techniques have been proposed to automatically infer software behavioral models. These techniques either (1) infer model (mainly as a finite state automata (FSA)) that generalize the observed invocation sequences found in interaction traces (e.g.,~\cite{lo:2009,lo:2006a,lorenzoli:2008}) or (2) identify high level properties - declarative class and method invariants - by observing how the state (internal variable) if a system is changing at runtime (e.g.,~\cite{beschastnikh:2011,beschastnikh:2013}). In this paper, we focus on inferring system model as a FSA, namely techniques that generate FSA from interaction traces to capture valid invocation sequences. FSA has sequence, alternation and repetition (i.e., loop and cycle) constructs to represent the behavior of a system.

While existing research on FSA-based behavioral model inference have made substantial contributions, they also have had significant limitations, i.e., their inferred models are often overgeneralized. Many of these approaches \cite{lo:2006a,lo:2006b, lo:2009,lorenzoli:2008,reiss:2001, walkinshaw:2008,cook:1998} have adopted kTail algorithm \cite{biermann:1972} with some extension. Thus, all of them suffer in overgeneralization problem related to kTail's state merging principles/heuristics - (1) in kTail the state merging is based on local behavior of states, i.e., it merges two states only by looking \textit{k} future consecutive sequence of operations, thus, it can lead to imprecision, when states share their next future but differ in their distant future (and even satisfies temporal invariants), and (2) kTail starts with inter-trace state merging rather than intra-trace state merging, thus, can fail to spot a generalization clue demonstrates in a trace. Recently, a new technique has been proposed, called Synoptic \cite{beschastnikh:2011, schneider:2010} that infers model similar to a FSA model. Synoptic starts with a coarse initial model, and then refines it to satisfy only three types/kinds of temporal invariants among many other possible types of invariants. Moreover, temporal invariants cannot guarantee to capture system constraints completely. Thus, Synoptic overgeneralizes in many cases where the considered three temporal invariants are limited to capture necessary constraints.

As a consequence of overgeneralization, their inferred models include many spurious behaviors that hinder the effectiveness of down-stream analysis techniques. In a study, Lo et al. show that automata learners generate imprecise and overgeneralized models especially when models are large and complex~\cite{LO20122063}. Overgeneralized models produce many false positives that significantly reduce the effectiveness of software emulation, verification and validation techniques.

In this paper, we present a technique to infer more precise system model as a FSA by using a set of heuristics. The basis of our inference technique is heuristic based generalization and truthful minimization. We generalize each individual traces based on our insight that a trace can be thought of as a separate path in a finite state machine, and thus can provide an indication of a potential general behaviour of a system, which can be deduced with high precision based on additional evidences observed in other traces. The intuition of our heuristics is that a set of valid sequence of operations of a system observed in its traces exhibits evidence to generalize the system behavior. Even though the repetition of FSA has infinite number of possible sequences of operations, we argue that for a real software system model, however, we can infer potential repetition behavior based on a number of recurrences of related operations with particular order observed in system traces. As the count of recurrence value is higher, the stronger the evidence and thus enhance the precision. We provide a control on the level of evidence by allowing users to set the count of recurrence. Finally, we combine generalized trace model by applying truthful state merging technique that makes our model concise without imposing spurious behavior.

==> problem.tex <==
\section{Problem Description}
\label{sec:problem}
Given a set of traces, the behavioral models mining problem can be stated as: \textit{mine a behavioral model which is as close as possible to the actual behavioral model of the system}.

Let us consider a set of traces :
\begin{table}[h]
	\centering
	\caption{Example Traces}
	\label{tab:exampletraces}
	\begin{tabular}{cc}
	\hline 
	No.  & Trace  \\ \hline
	1 &  <regLogin,order,inv,pay,ship>  \\\hline
	2 & <premLogin,order,ship,inv,pay> \\\hline
	3 & <premLogin,cata,cata,order,ship,inv,pay> \\\hline
\end{tabular}
\end{table}

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.15\textwidth]{figures/flowermodelretailerservice}
	\caption{\small{Flower model for \emph{retailer} service}}
	\label{fig:flowermodelretailerservice}
\end{figure}

Consider the extreme case of the concise/generalize model, illustrated in Figure \ref{fig:flowermodelretailerservice}. This model is overgeneralized because it accepts conversations that are absent on the real model and, in fact, accepts all possible conversation consisting of retailer service messages. While only a subset of the possible conversations formed from these operations actually present on the real model (see Figure \ref{fig:retailerservice}).

At the other extreme case of the precise/accurate model, it is possible to build a model with a path from each distinct conversation of the log (also referred to as prefix tree acceptor (PTA)). A PTA is a tree representation of a set of traces. Each trace corresponds to a path in the tree. The PTA is obtained by merging the initial states of each trace into a single initial state, and from that state, merging all those states that are reached by the same invocation sequence. Traces that share the same prefix, share also a sub-path in the tree. Figure \ref{fig:ptamodelretailerservice} shows a PTA for three traces. Such model would be difficult to understand, having too many states. Moreover, it is too \emph{precise}, i.e., \emph{undergeneralized}, since it accepts only the conversations in the log that usually reflect a partial behavior of the real model. 

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/ptamodelretailerservice}
	\caption{\small{PTA model for example traces of Table \ref{tab:exampletraces}}}
	\label{fig:ptamodelretailerservice}
\end{figure}

There are two possible strategies, so far, have been proposed in the literature to balance the trade-off between overgeneralization and undergeneralization (see section~\ref{sec:related work} for a detail literature review): \textit{k-equivalence state merging} and \textit{invariant (temporal) enhanced state merging}.

\subsection{k-equivalent state merging}
The k-equivalent state merging, i.e., kTail approach \cite{biermann:1972} captures the intuitive idea that if two states are not distinguishable by looking to their near future, they probably represent the same conceptual state, and thus can be merged. The kTail algorithm relies on selecting an appropriate \textit{k}. This choice typically involves a trade-off between \textit{precision} (smaller \textit{k} implies more spurious merges due to the limited ``scope" and thus \textit{overgeneralized}) and \textit{recall/completeness} (larger \textit{k} implies fewer merges, and thus \textit{undergeneralized}) of the generated model. For instance, if we apply kTail algorithm with \textit{k}=1 on trace1 and trace2 of Table \ref{tab:exampletraces}, it merges state q3 with q9, q4 with q7, and q1 with q6 and infers imprecise model shown in Figure \ref{fig:ktailwithk=1}. It allows lot of spurious behaviors include \textit{<premLogin, order, inv, pay>, <regLogin, order, ship>}, where transaction completed without shipment and without payment respectively. If we apply, kTail with k=2, the algorithm merges state q2 of trace1 to q8 of trace2 of the PTA model in Figure \ref{fig:ptamodelretailerservice}. The resulted infer model will be as shown in Figure \ref{fig:ktailwithk=2}. Even though the newly inferred model is more precise than 1-Tail model, it still allows spurious behaviors as shown in Table \ref{tab:spuriousmodel}.  

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/ktailwithk=1}
	\caption{\small{Inferred model using kTail (k=1) for trace1 and trace2}}
	\label{fig:ktailwithk=1}
\end{figure}

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/ktailwithk=2}
	\caption{\small{Inferred model using kTail (k=2) for trace1 and trace2}}
	\label{fig:ktailwithk=2}
\end{figure}

\begin{table*}[h]
	\centering
	\caption{Spurious behaviors of kTail inferred model}
	\label{tab:spuriousmodel}
	\begin{tabular}{cc}
		\hline 
		Trace  & Description  \\ \hline
		<premLogin, order, inv, pay> &  Transaction ended without shipment  \\\hline
		<regLogin, order, inv, pay> & Transaction ended without shipment \\\hline
		<premLogin, order, ship, inv, pay, ship> & Allows two shipments for a single order of premium customer \\\hline
	\end{tabular}
\end{table*}

\subsection{Invariant enhanced state merging}
To reduce overgeneralization/imprecision, Lo et al. \cite{lo:2009} proposed kSteering that extends kTail by using temporal invariants inferred from traces to steer the generation of FSA. The authors consider future-time and past-time temporal rules to prevent state merging that breaks non-local relations and thus improve the precision of the inferred FSA. Future-time temporal rules, e.g., e1->e2, specify relations of the type ``whenever an event (say e1) happened (pre-condition) another event (say e2) must eventually happen (post-condition)''. Past-time temporal rules, e.g., e1<-e2, specify relations of the type `Whenever an event (say e2) happened (pre-condition), another event (say e1) must have happened before (post-condition)".

kSteering prevents to merge states of two traces if their future operation sets (i.e., the operation sets of these traces starting after state merging point to end) are different from each other in terms of \textbf{operation names}. Let us consider that \textit{<s, m, a, b, n, f>} and \textit{<s, u, a, b, v, f>} are two traces, as shown in figure \ref{fig:kSteeringExampleTraces}. The kSteering can successfully prevents merges state q2 to q9 and q3 to q10, as the inferred temporal rules, \textit{m->n, m<-n, u->v} and \textit{u<-v} do not comply the merge. However, it can not handle spurious merges if the operation sets are same in terms of names but differ in sequences. For example, the kSteering can not prevent the spurious merges in trace1 and trace2 (Table \ref{tab:exampletraces}) as the inferred temporal rules (see Table \ref{tab:inferredtemporalrulesksteering}) are not violating for k-equivalence merges (k=1,2). 
\begin{figure}[tb]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/kSteering-example-traces}
	\caption{\small{Example traces}}
	\label{fig:kSteeringExampleTraces}
\end{figure}

\begin{table}[h]
	\centering
	\caption{Inferred temporal rules by kSteering}
	\label{tab:inferredtemporalrulesksteering}
	\begin{tabular}{c|c}
		\hline 
		Future-time   & Past-time   \\ 
			temporal rules  & 	temporal rules  \\		\hline
		regLogin->order, regLogin->inv,  &  order<-inv,   \\
		regLogin->pay, premLogin->order,  & order<-pay,   \\
		premLogin->ship, premLogin->inv, &   order<-ship,    \\
		premLogin->pay, order->inv,  &      inv<-pay  \\
		order->pay, order->ship, inv->pay  &     \\
		\hline
	\end{tabular}
\end{table}

==> relatedwork.tex <==
\section{Related Work}
\label{sec:related work}
There have been numerous work in the area of specification/behavior mining. They can be classified into two groups, depending on what the mined specifications represent: order of events (e.g.,~\cite{lo:2009}) and invariants on values of program variables (e.g.,~\cite{beschastnikh:2011}).

\subsection{Mining models of ordered events}
\subsubsection{FSA-based Model}
There are many simple FSA learners []. The approach ranges from passive (i.e., only analyse execution traces) to active (i.e., ask queries to users or generate test cases such as []). These learners also analyse different kind of execution traces, from standard program execution traces to network traces ([]), WSDL descriptions ([]), and system logs ([]).
The kTail algorithm \cite{biermann:1972} serves as a basis for many approaches for mining FSA models from invocation traces []. These approaches extend kTail to (1) improve its precision or recall [], (2) incrementally generate a FSA [kBehaviour], (3) build larger frameworks with kTail as the inference algorithm [], and (3) enhance the models with information about invocation probabilities [] and program state and method parameters []. These approaches extend kTail mainly by either considering (1) trace invariants \cite{lo:2009} or (2) values of method parameters \cite{lorenzoli:2008} [KLFA]\cite{krka:2014}, in addition to kTail. As all of these approaches have adopted kTail algorithm with some extension, thus the key limitation of kTail's principle, i.e., inter-trace state merging, also applies to these approaches.

Synoptic \cite{schneider:2010, beschastnikh:2011} uses the CEGAR \cite{clarke:2000} approach to create a coarse initial model, and then refine it using counter examples that falsify temporal invariants. Even Synoptic represents model as a graph, we discuss it here as the graph model can easily be converted to an equivalent FSA model. Meanwhile, InvariMint \cite{beschastnikh:2013} presents a declarative specification language for expressing model-inference algorithms, and improves the efficiency of algorithms, but neither their precision or recall. 

\subsubsection{Non FSA-based Model}
Although FSA are a popular model, there are many technique to learn other models that describe the order of events, like sequence diagrams, frequent pattern and temporal properties. In general, different models capture different aspects and are thus mutually complementary.

Many techniques for mining sequence diagrams simply represent traces as sequence diagrams []. Some of these techniques can also infer loops [] or modalities []. Some techniques can infer patterns or sequence of events that repeat frequently in a set of traces []. There are also several techniques to mine temporal properties. Yang et al. present an approach to mine two-event future-time temporal logic rules, which are significant with respect to a user-defined satisfaction rate []. Lo et al. extended this work to mine significant future-time temporal rules of arbitrary lengths []. In further work, Lo et al. propose a method to mine significant past-time rules of arbitrary lengths [].

In our work, we produce FSA as a final result. FSA can describe a more complete relations between events as compared to frequent patterns and temporal rules. Frequent patterns only capture some linear relations between events that appear frequently. Temporal rules describe a partial relations between events and cannot completely capture loops and branches. The more complete relations among events can be a very useful input to many testing and analysis techniques.

\subsection{Mining models of invariants on values of program variables}
Different from the goal of this work, there are several techniques that mine behavioural models of invariants on values of program variables. These models usually represent aspects that complement the information described by FSA. The most popular example is Daikon, a mining approach to learn boolean expressions that describe likely invariants on values of program variables \cite{ernst:2001}. Similar to Daikon, Contractor technique \cite{de:2012} creates models based solely on the inferred state invariants. Contractor++ [] addresses the limitations of Contractor when applied to dynamically inferred, as opposed to manually specified, state invariants. TEMI \cite{krka:2014} infers models from invariants and then enhances them with execution traces. The first phase conceptually similar to Contractor++, capturing all invocation sequences of a system allowed by the invariants. The second phase promotes transitions observed in the traces from maybe to required.


==> specminer.tex <==
\section{SpecMiner Framework}
\label{sec:specminerframework}
In this section, we give an overview of our proposed approach and then present it in details.
\subsection{Overview}
The goal of our approach is to infer a general system model without compromising accuracy. A trace is a sequence of operations and can be represented as a FSA with exactly one path. Thus, to generalize a set of traces, it is required to merge the states of the FSAs. We propose intra-trace state merging unlike other approaches such as kTail that does inter-trace state merging. Intuitively, a trace gives an insight of a system behavior. Thus, we argue that merging the states in a trace-level will enhance the accuracy of generalization. 

As shown in Figure \ref{fig:SpecMinerapproachoverview}, SpecMiner approach works in two phases: (1) heuristic-driven generalization and (2) automata minimization. 


\begin{figure}[htb]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/overview}
	\caption{\small{SpecMiner approach overview}}
	\label{fig:SpecMinerapproachoverview}
\end{figure}

\subsection{Heuristic-driven Generalization}
\label{subsec:heuric-driven generalization}
We propose a set of heuristics that serve as evidences for generalization and guide the generalization process. We propose these heuristics for each of the generalization properties (i.e., cycle, loop and multi-loop) of FSA by analysing their corresponding distinctive patterns that appear in traces. Below we present those heuristics for each of the generalization properties.
\subsubsection{Loop}
If a system model has a loop, we expect a trace with consecutive repetition of the loop operation. The repeat value/ frequency/count (RC) \textit{n} is an integer number, where \textit{n}>=2. Repeat value equal 1 cannot be used to identify loop as it is similar as sequence. For most of the system value 2 is enough to precisely identify loop, i.e., to overcome overgeneralization. However, there could be a special case, for instance, the login example presented in Figure \ref{fig:loginex} (a system that allows maximum four incorrect login attempts before blocking an account and enforcing users to answer security questions to proceed further). In that case, we need to set repeat count 5. It is good to set the count as high as we can but it is required to make sure that at least one trace exists with such number of repeated loop operation.
\begin{figure}[htb]
\centering
\includegraphics[width=0.48\textwidth]{figures/loginex}
\caption{a partial system model that asks for security information after four incorrect login attempts}
\label{fig:loginex}
\end{figure}

Figure \ref{fig:loopheuristic} shows three different generalized FSA model for a loop and their corresponding representative traces (a set of traces uses as an evidence to support generalization). Given a base trace \textit{<prefix, a, a, a, a, suffix>} and \textit{RC} equal 2, there are three possible general models as shown Figure \ref{fig:loopheuristic}. The ultimate general model depends on the other representative traces, called supportive traces. The FSA model shown in Figure \ref{fig:loopheuristic}a will be the final general model if the supportive trace \textit{<prefix, suffix>} founds valid, i.e., it presents on the input traces. If we found the supportive trace \textit{<prefix, suffix>} is an invalid trace, we search for new supportive trace \textit{<prefix, a, suffix>} and linearly increase the number of loop operation in the supportive trace until \textit{|base-trace - support-trace|>= RC}. In this example, the value of \textit{|base-trace - support-trace|} reaches 2 for case3 and if the trace \textit{<prefix, a, a, a, suffix>} cannot be found in input traces, we treat \textit{<prefix, a, a, a, a, suffix>} as just a sequence of transition without any generalization. We do not further proceed to consider \textit{<prefix, a, a, a, suffix>} as a supportive trace because for it the value of \textit{|base-trace - support-trace|} less than RC, i.e., 1.

\begin{figure*}[tb]
	\centering
	\includegraphics[width=1.00\textwidth]{figures/loop}
	\caption{\small{Heuristic for a loop}}
	\label{fig:loopheuristic}
\end{figure*}

\subsubsection{Multi-loop}
It is a special case of (single) loop where a state contains two or more loops. In this case, we need additional representative traces as evidence to support valid generalization. 

\subsubsection{Cycle}
If a system model has a cycle, we expect that there should be a trace with repetition (at least twice, i.e., RC=2) of the cycle. For example, the trace \textit{<prefix, a, b, c, a, b, c, suffix>} shows a possibility of cycle related to the sequence of operations \textit{<a, b, c>} which we can further confirm by checking whether the trace \textit{<prefix, suffix>} is valid or not. If valid, the generalization would be as shown in Figure \ref{fig:cycleheuristic}a. A presence of subsequent cycle operations before suffix, in this example {a} or {a, b}, requires a slight variation of generalization as shown in Figure \ref{fig:cycleheuristic}b and \ref{fig:cycleheuristic}c. 

\begin{figure*}[tb]
	\centering
	\includegraphics[width=1.00\textwidth]{figures/cycle}
	\caption{\small{cycle generalization heuristic examples}}
	\label{fig:cycleheuristic}
\end{figure*}
An extra checking is required if the number of operations in the cycle is 2. For example, the trace \textit{<prefix, a, b, suffix>} is valid for both the models in Figure \ref{fig:cycleSpecialCase}, however these models are not equivalent. To precisely identify the final model, we need additional representative trace to check further. In this case, for instance, if the trace \textit{<prefix, suffix>} is found as a valid trace (i.e., it exits in input traces), we take the model shown in Figure \ref{fig:cycleSpecialCase}a as our generalized model. If the trace \textit{<prefix, a, b, suffix>} is found as a valid trace, our generalized model would be as shown in Figure \ref{fig:cycleSpecialCase}b.

\begin{figure*}[htb]
	\centering
	\includegraphics[width=0.85\textwidth]{figures/cycle-specialcase}
	\caption{\small{Heuristic for a loop}}
	\label{fig:cycleSpecialCase}
\end{figure*}

\subsubsection{Nested Cycle}
Nested cycle is defined as cycle(s) within a cycle. Let consider the traces R1a, R1b and R1c corresponds to the reference model in Figure \ref{fig:nestedcycleheuristic}a. If we apply the cycle heuristic as explained above in the trace \textit{<prefix, a, b, c, a, b, c, a, m, n, m, n, suffix>}, it results a generalized model as shown in Figure \ref{fig:nestedcycleheuristic}b which is an overgeneralization related to model in Figure \ref{fig:nestedcycleheuristic}a. This overgeneralization occurs because of making a cycle (for m, n) in a state (here s1) which is already a part of another cycle (a, b, c). In this case, our generalization will be as shown in Figure \ref{fig:nestedcycleheuristic}a.
For a model with nested cycle as shown in Figure \ref{fig:nestedcycleheuristic}b, we expect a trace R1b \textit{<prefix, a, b, m, n, m, n, c, a, b, m, n, m, n, c, a, suffix>} should exist on input traces. First we find the largest repeated substring (as underlined in the trace R1b) that indicates cycle. Trace R2b provides further support the existence of cycle. In the same way, iteratively, we check the existence of a repeated substring in a substring.

\begin{figure*}[htb]
	\centering
	\includegraphics[width=0.85\textwidth]{figures/nested-cycle}
	\caption{\small{Nested cycle examples}}
	\label{fig:nestedcycleheuristic}
\end{figure*}

\subsubsection{Loop within cycle}
It is loops(s) within a cycle. We address this case in the similar way to nested cycle. Figure \ref{fig:loopwithincycle}a presents how we overcome overgeneralization that causes if we apply Loop and cycle heuristics as explained above without further consideration. Figure \ref{fig:loopwithincycle}b presents an example of loop within cycle model and the required representative traces to infer that model.

\begin{figure*}[htb]
	\centering
	\includegraphics[width=0.85\textwidth]{figures/loop-within-cycle}
	\caption{\small{Loop within cycle}}
	\label{fig:loopwithincycle}
\end{figure*}

\subsection{Minimization}
The resulting FSA from generalization process will be non-deterministic, i.e., there exist more than one path from initial state for a given operation name. We employ the non-deterministic FSA to deterministic FSA (i.e., for a given operation name there can exist only one path from a state) conversion before applying minimization. This process may cause the generation of equivalent states, i.e., they have the same outgoing transitions, which means that they can be merged without changing the FSA properties. Indeed, merging equivalent states allows minimizing the FSA without changing the set of conversations it accepts. We use the Ullman-Hopcroft minimization algorithm \cite{hopcroft:2001} for this purpose.  

\subsection{Inference Algorithm}

\begin{algorithm*}[htb]
	\caption{Inference Algorithm}\label{alg:InferenceAlgorithm}
	\begin{algorithmic}[1]
		\STATE \textit{Input:} set of traces, \emph{T} = $(t_1,..., t_n)$ where $t_i$ is a valid sequence of operations $<op_1, op_2,..., op_k>$ with $t_i[1]=op_1$ and $t_i[t_i.length]=op_k$, minimum repeat count \emph{RC}$\geq$0, depth count \emph{DC}$\geq$0
		\STATE \textit{Initialize:}  \emph{FSA} = \emph{start node}
		\STATE \textit{Output:} FSA
		
		
		\FOR {$t \in T$}
		\STATE $tFSA \leftarrow$ initialize $FSA$ with start node
		\FOR{$index \in \{1,\dots,|t|\} $}
		\IF {\textit{a sequence of operations $OP\in t$ consecutively repeated at least RC times 
				starting from $t[index]$}}
		\STATE Create Representative Traces (RT) based on $|OP|$, $t.prefix$, $t.cycOP$ and $t.suffix$ 
		
		\IF {$RT \in T$}
		\STATE $cFSA \leftarrow$ SpecMiner($OP, RC, DC$)   %changed its position
		\STATE $tFSA \leftarrow$ add $cFSA$ as a cycle
		\STATE $index \leftarrow$  $index +|cycle|$
		\ELSE
		\STATE $tFSA \leftarrow$ add $cFSA$ as a sequence of transitions
		\STATE $index \leftarrow$  $index +|OP|$
		\ENDIF 
		\ELSE 
		\IF {\textit{the operation t[index] consecutively repeated at least RC times 
				starting from $t[index]$}}
		\IF {\textit{the current state of $tFSA$ contains a loop and the representative 
				traces for multiloop (created based on $DC$ value) are found in $T$, i.e., 
				$RT \in T$}}
		\STATE $tFSA \leftarrow $ add a loop transition with name $t[index]$
		\ENDIF
		\IF {\textit{the current state of $tFSA$ contains a cycle and the 
				representative traces for loop within cycle are valid}}
		\STATE $tFSA \leftarrow $ add a transition followed by a loop with name $t[index]$
		\ENDIF
		\IF {\textit{the representative traces for loop are valid}}
		\STATE $tFSA \leftarrow $ add the operation $t[index]$ as a sequence of transitions and loop
		\ELSE
		\STATE $tFSA \leftarrow $ add the operation $t[index]$ as a sequence of transitions 
		\ENDIF
		\STATE $index \leftarrow $ $index+ |loop|$
		\ELSE
		\STATE $tFSA \leftarrow$ create a new state with a transition name $t[index]$
		\STATE $index \leftarrow$  $index +1$
		\ENDIF
		\ENDIF
		%\STATE dfdsf
		\ENDFOR
		\ENDFOR
		\STATE $FSA \leftarrow $ ConvertNFAtoDFA($tFSA$)
		\STATE $FSA \leftarrow $ Minimize($FSA$)
		\STATE Return $FSA$	
		
	\end{algorithmic}
\end{algorithm*}

Our proposed heuristics for generalization are presented in section \ref{subsec:heuric-driven generalization}. This section presents our inference algorithm to infer a FSA based system model  from a set of traces with the given repeat count and depth count value. For each of the input trace (line 4), starting from the first operation to its end (line 6), the algorithm considers the operation sequence to identify whether the consecutive operations depicts the behavior of cycle (line 7) or loop (line 18). If cycle it applies heuristics related to cycle as described in section \ref{subsec:heuric-driven generalization} (line 8 to 16). The algorithm first identifies repeated operations set, prefix and suffix, and accordingly creates representative traces (line 7 and 8). If these representative traces found valid (line 9), the algorithm is called recursively (line 10) by sending the repeated operation set as a trace to address nested cycle and/or loop within cycle cases. The resulted cFSA could be a simple FSA with a sequence of transitions (in case no inner loop or cycle) or a complex FSA (i.e., contains cycle and/or loop). Based on the prefix and suffix values, we incorporate this cFSA with tFSA as a cycle (line 11) (see Figure \ref{fig:cycleheuristic} for example). After that index of the trace is incremented to the position of operation that will be considered next (line 12). If the representative traces found invalid, we incorporate cFSA to tFSA as a sequence of transitions without cycle (line 14).

If an indication of loop is shown (line 18), we create and validate representative traces to identify whether it is a case of multiloop (line 19) or loop within cycle (line 22) or simple loop (line 25) or not even loop (line 27), and generalize the trace accordingly. Once the generalization is completed for a trace, we  convert the final FSA (line 38) to DFA and minimize it (line 39).



==> threat.tex <==
\section{Threats to validity}
\label{sect:threat}
In this section, we outline the possible threats to our evaluation's validity and discuss our mitigation strategies.
\subsection{Ground-truth bias}
The ground-truth models were manually constructed. This may make them biased to the specifier's expertise. To mitigate this threat, we used the publicly available ground-truths from other researchers.
\subsection{Subject libraries}
The selection of libraries may bias the evaluation results. For instance, models of a well-known library may not be representative of dynamically inferred models in general. Thus, we selected libraries from different domains and of various sizes. 
\subsection{Metrics} 
There are multiple ways of comparing the generated models with the corresponding ground-truth models (e.g., recall and precision of the simulated traces vs. graph comparison), which could potentially yield different results. Our mitigation strategy used metrics that have been proposed and adopted by the research community [], and are consistent with our goal of comparing model behaviour, not structural similarity.

